Fine Grained Dataflow Tracking with Proximal Gradients

Dataflow tracking with Dynamic Taint Analysis (DTA) is an important method in systems security with many applications, including exploit analysis, guided fuzzing, and side-channel information leak detection. However, DTA is fundamentally limited by the Boolean nature of taint labels, which provide no information about the significance of detected dataflows and lead to false positives/negatives on complex real world programs. We introduce proximal gradient analysis (PGA), a novel, theoretically grounded approach that can track more accurate and fine-grained dataflow information. PGA uses proximal gradients, a generalization of gradients for non-differentiable functions, to precisely compose gradients over non-differentiable operations in programs. Composing gradients over programs eliminates many of the dataflow propagation errors that occur in DTA and provides richer information about how each measured dataflow effects a program. We compare our prototype PGA implementation to three state of the art DTA implementations on 7 real-world programs. Our results show that PGA can improve the F1 accuracy of data flow tracking by up to 33% over taint tracking (20% on average) without introducing any significant overhead (<5% on average). We further demonstrate the effectiveness of PGA by discovering 22 bugs (20 confirmed by developers) and 2 side-channel leaks, and identifying exploitable dataflows in 19 existing CVEs in the tested programs.

==> sections/working_example.tex <==
%-------------------------------------------------------------------------------
\subsection{Working Example}
%-------------------------------------------------------------------------------
\begin{comment}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\linewidth]{figs/sosp-working_ex3}
    \caption{\label{fig:working_ex1}Proximal cost function at $\bar{x} = 7$.}
  \end{subfigure}
  \hspace{0.1cm}
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\linewidth]{figs/sosp-working_ex2}
    \caption{\label{fig:working_ex2}Evaluated Proximal Gradient for $\bar{x} = 7$.}
  \end{subfigure}
  \vspace{-15pt}
  \caption{\label{fig:working_ex}Example of Proximal Gradient Evaluation.}
  \vspace{-15pt}
\end{figure}
\end{comment}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/sosp-grad_v_taint_ex}
  \vspace{-25pt}
  \caption{\label{fig:taint_v_gradient} Example of a program in which an iterated shift operation on the input will cause overtainting, while gradient will correctly identify which input bytes are most influential for the given sync (cur\_input).}
  \vspace{-15pt}
\end{figure}

To give a better intuition for how proximal gradients work in practice, we provide a working example. Consider the function $f(x) =   x \texttt{\&} 4$ shown in figure \ref{fig:ex_funcs}, and suppose we are evaluating it with $\bar{x} = 7$. This type of bitwise operation is common in programs that parse a file for input, since they frequently need to check if flag bits are set in a header or section header of the file. However, discrete functions like bitwise operations are nondifferentiable so we instead evaluate the proximal gradient.

To evaluate the proximal gradient on $f\left(x\right)$, the sampling region must first be defined. \tc{x \& 4} has a Lipschitz Constant of $K=4$ (any bitwise operation with a constant has a Lipschitz Constant with the value of the most significant bit in the constant), so assuming a proximal scaling factor of $\lambda = 1$, the sampling distance bound is $2K = 8$. Therefore, a total of 16 samples must be taken, for $x = [-1, 15]$, and the cost function of the proximal operator, $f(x) + ||x - \bar{x}||_2^2$ evaluated for each possible $x$. Figure \ref{fig:working_ex1} shows the value of the cost function near $x = 7$, there is a clear minimum at $x=8$, where $f\left(8\right) + ||8-7||_2^2 = 1$, so the proximal operator evaluates to $x=8$. The proximal gradient is then $prox_{\nabla f}\left(7\right) = \frac{f\left(7\right) - f\left(8\right)}{7 - 8} = -4$.



